Supporting Multiparty Signing over Named Data Networking

Modern digitally controlled systems require multiparty authentication and authorization to meet the desired security requirement. This paper describes the design and development of NDN-MPS, an automated solution to support multiparty signature signing and verification for NDN-enabled applications. NDN-MPS suggests several changes and extensions to the existing NDN security solutions. First, it introduces a new type of trust schema to support signing and verification for multiple signers under complex policies such as threshold schemes. Second, it extends the NDN signature format to accommodate multisignature schemes such as BLS signature. Third, it introduces a signature collection protocol to solicit signatures securely from multiple signers. We further evaluate NDN-MPS by assessing its security properties and measuring its performance.

==> sections/imple.tex <==
\section{Implementation}
\label{sec:imple}

We have implemented \sysname into an open-source library~\footnote{The codebase repository URL will be included with the final version of the paper} in C++.
Our library depends on ndn-cxx~\cite{ndn-cxx} and a BLS library~\cite{herumi-bls} that have been fully examined and is compatible with the BLS API specification defined by Ethereum 2.0~\cite{ethereum2-bls}.
Our library is implemented over the curve BLS12-381.
In this section, we explain our implementation of multiparty trust schema and the integration of \sysname into NDNCERT to realize multiparty-approved certificate issuance and revocation.


%\subsection{Implementation of Encoding}
%
%\sysname implements the encoding of the signature in NDN interest and data, as well as the encoding for the signers list.
%The cryptographical operations and serialization of BLS signature and keys are provided by BLS library \cite{herumi/bls}.
%The implementation is built over NDN-CXX, which comes with capability for key management and signing.
%Even though \sysname extends NDN-CXX's capability with another type of key and signature, the library uses a separate data structure for maintain the BLS key and signatures.
%However, both kind of signature are encoded the same way, except that BLS signatures have a different signature type.
%Therefore, the \sysname library needs distingish the type of signature using this signature type label, and process the key and signature using the corresponding library function.
%
%The team also tried modifying NDN-CXX to support BLS signatures directly, but doing this would make existing NDN-CXX code and libraries incompatible to the new \sysname library.

\subsection{Multisignature Trust Schema Implementation}
\label{sec:schema-impl}
\label{sec:imple:schema}

The multisignature trust schema is implemented in the library as a trust schema configuration file parser.
To support more complicated use cases where there are multiple acceptable signer sets, one can simply created multiple trust schema files applying to the same data prefix.
In the signature verification process, the signature is accepted if there is at least one trust schema rule is satisfied.
The known signers are implemented with a separate configuration file which contains a list of NDN certificates.

\subsection{Multiparty Certificate Management}

As a use case, we have integrated the \sysname into an NDN certificate management system, NDNCERT~\cite{ndncertposter}.
To be more specific, we add a new type of authentication verification challenge that is based on multiple parties' approval.
When a user is requesting a new certificate or trying to revoke an existing certificate from a certificate issuer, the new challenge allows the issuer to agree on user's request if the user can provide a multiparty signature signed by a sufficient set of signers.
In this scenario, the user needs to act as the coordinator to decide the signer set, collect and aggregate signature pieces from the signers following the \sysname protocols.
After that, in the Challenge phase of the NDNCERT protocol, the user needs to submit the signed data along with the signature information packet to the certificate issuer.
The issuer in this case is the verifier of the data, who verifies the credential according to its trust schema, then generates the certificate if the prove is valid.
Similarly, this process can be used with the revocation of the certificate as well.

%Instead of the new issuer requesting the key, the party questing the revocation is responsibile to collect the signature.
%If it is able to collect enough votes or endorsement from other authoriative parties for revoking the certificate, it is able to aggregate and generate a multisigned proof data.
%This data can be used to prove the issuer that the revocation is legitimate.
%On revocation, this request is being logged into DLedger, a distributed ledger, with the revoked certificate information and the proof.
